FeatUp: A Model-Agnostic Framework for Features at Any Resolution

Deep features are a cornerstone of computer vision research, capturing image semantics and enabling the community to solve downstream tasks even in the zero- or few-shot regime. However, these features often lack the spatial resolution to directly perform dense prediction tasks like segmentation and depth prediction because models aggressively pool information over large areas. In this work, we introduce FeatUp, a task- and model-agnostic framework to restore lost spatial information in deep features. We introduce two variants of FeatUp: one that guides features with high-resolution signal in a single forward pass, and one that fits an implicit model to a single image to reconstruct features at any resolution. Both approaches use a multi-view consistency loss with deep analogies to NeRFs. Our features retain their original semantics and can be swapped into existing applications to yield resolution and performance gains even without re-training. We show that FeatUp significantly outperforms other feature upsampling and image super-resolution approaches in class activation map generation, transfer learning for segmentation and depth prediction, and end-to-end training for semantic segmentation.

==> tables/additional_baselines.tex <==
\begin{table}[h]
  \centering
  \renewcommand*{\arraystretch}{1.3}
    \begin{tabular}{r|cc|cc|cc|c}
    \hline
\multicolumn{1}{l|}{} & 
\multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}CAM\\ Faithfulness\end{tabular}}} & 
\multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Object\\ Localization\end{tabular}}} & 
\multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Semantic\\ Segmentation\end{tabular}}} & 
\textbf{\begin{tabular}[c]{@{}c@{}}Depth\\ Estimation\end{tabular}} \\
    % & & & & & & &     \\ % blank row
    \hline
    & A.D.$\downarrow$ & A.I. $\uparrow$ & GT \% $\uparrow$ & Top-1 \% $\uparrow$ & Acc. $\uparrow$ & mIoU $\uparrow$ & SSIMSE $\downarrow$ \\
    \hline
    Low-Res & 16.4 & 4.81 & 16.2 & 13.1 & 0.559 & 0.310 & 86.22 \\
    Bilinear & 13.6 & 5.00 & 16.5 & 13.5 & 0.607 & 0.367 & 78.87\\
    U-Net & 13.8 & 5.17 & 16.2 & 13.2 & 0.601 & 0.334 & 73.73 \\
    Strided & 24.4 & 2.00 & 14.4 & 10.8 & 0.595 & 0.348 & 80.02 \\
    Large Image & 35.9 & 1.04 & 14.2 & 9.91 & 0.597 & 0.355 & 104.2 \\
    \hline
    FastFeatUp & {\ul 11.6} & {\ul 5.39} & {\ul 17.0} & {\ul 13.8} & {\ul 0.610} & {\ul 0.368} & {\ul 68.10} \\
    FeatUp & \textbf{9.47} & \textbf{5.59} & \textbf{17.8} & \textbf{14.2} & \textbf{0.621} & \textbf{0.383} & \textbf{66.12} \\
    \hline
  \end{tabular}
        \vspace{.15in}

  \caption{Comparison of feature upsamplers across a variety of downstream tasks. FeatUp and FastFeatUp consistently outperform baselines, including the learned U-Net and large feature map obtained from a higher-resolution input image.}
  \label{tab:main_results}
      \vspace{-.15in}
\end{table}

==> tables/cuda_benchmark.tex <==
\begin{table*}[t]
\begin{center}

\begin{tabular}{ccccc}
Shape (B, H, W, C, F)  & Method & Forward (ms) & Backward (ms) & Peak Mem (Mb) \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{$1 	\times 14 \times 14 \times 2048 \times 5$}} & Ours & \textbf{0.15} & \textbf{1.05} & \textbf{6.24} \\
\multicolumn{1}{c|}{}                                                               & TorchScript & 2455          & 69367         & 12.8          \\
\multicolumn{1}{c|}{}                                                               & Unfold      & 3.30          & 2.81          & 119.          \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{$1 	\times 512   	\times 512 	\times 3 	\times 5$}}   & Ours        & \textbf{0.55} & \textbf{2.10} & \textbf{10.2} \\
\multicolumn{1}{c|}{}                                                               & TorchScript & 147.          & 520.          & 24.3          \\
\multicolumn{1}{c|}{}                                                               & Unfold      & 3.47          & 4.85          & 231.          \\ \hline
\end{tabular}

\caption{Comparing the performance of our CUDA JBU kernel with implementations based on PyTorch's \texttt{Unfold} operation and TorchScript. Our implementation dramatically reduces memory overhead and increases inference speed. Additional experiments and details can be found in the Supplement.}
\vspace{-5px}
\label{tab:cuda_benchmark}
\end{center}
\end{table*}

==> tables/probe.tex <==
% \begin{table}[]
% \begin{center}

% \begin{tabular}{l|cc|c}
%                & \multicolumn{2}{c|}{\textbf{Semantic Segmentation}} & \textbf{Depth}   \\
%                & \textbf{Accuracy}     & \textbf{mIoU}      & \textbf{SSIMSE}  \\ \hline
% Low-Res        & 0.6096                & 0.3276             & 8715.8          \\
% Bilinear       & 0.6441                & 0.3601             & 7915.4          \\
% Strided        & 0.6244                & 0.3405             & 8058.3          \\
% 2x Image       & 0.6398                & 0.3552             & 16777.          \\
% FPN       & 0.6281           & 0.3476        & 7573.3          \\
% \textbf{FFU}            & 0.6465                & 0.3630             & 7742.5          \\
% \textbf{FFU + MLP}      & \textbf{0.6741}       & \textbf{0.3929}    & 7646.2          \\
% \textbf{FFU + LG}       & {\ul 0.6729}          & {\ul 0.3928}       & 7334.4          \\
% \textbf{FFU + MLP + LG} & 0.6722                & 0.3905             & {\ul 7326.1}    \\
% \textbf{FeatUp}         & 0.6604                & 0.3775             & \textbf{7157.2}
% \end{tabular}
% \caption{Results of linear probe transfer learning on semantic segmentation and depth estimation. Our methods (bolded) consistently outperform baselines in both tasks.}
% \label{tab:probe}
% \end{center}

% \end{table}

==> tables/wsol_vit.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\centering
\begin{tabular}{l|cc}
\multicolumn{1}{c|}{} & \multicolumn{2}{c}{\textbf{CAM}}   \\
\multicolumn{1}{c|}{} & \textbf{GT \%} & \textbf{Top-1 \%} \\ \hline
Low-Res               & 39.62          & 30.01             \\
2x Image              & 36.59          & 27.35             \\
Strided               & 34.72          & 27.18             \\
FPN                   & 37.29          & 29.00             \\
FFU                   & \underline{48.72}    & \underline{37.27}       \\
FeatUp                & \textbf{53.85} & \textbf{41.29}   
\end{tabular}
\caption{WSOL performance on the CUB dataset, with features obtained from a ViT trained in a supervised manner. FeatUp outperforms existing baselines, with a +35.9\% GT and +37.6\% Top-1 Accuracy increase over the low-res features. FastFeatUp follows close behind as a lighter-weight replacement for FeatUp.}
\label{tab:wsol_vit}
\end{table}
